Unveiling Transformers with LEGO: a synthetic reasoning task

We propose a synthetic reasoning task, LEGO (Learning Equality and Group Operations), that encapsulates the problem of following a chain of reasoning, and we study how the Transformer architectures learn this task. We pay special attention to data effects such as pretraining (on seemingly unrelated NLP tasks) and dataset composition (e.g., differing chain length at training and test time), as well as architectural variants such as weight-tied layers or adding convolutional components. We study how the trained models eventually succeed at the task, and in particular, we manage to understand some of the attention heads as well as how the information flows in the network. In particular, we have identified a novel \emph{association} pattern that globally attends only to identical tokens. Based on these observations we propose a hypothesis that here pretraining helps for LEGO tasks due to certain structured attention patterns, and we experimentally verify this hypothesis. We also observe that in some data regime the trained transformer finds ``shortcut" solutions to follow the chain of reasoning, which impedes the model's robustness, and moreover we propose ways to prevent it. Motivated by our findings on structured attention patterns, we propose the LEGO attention module, a drop-in replacement for vanilla attention heads. This architectural change significantly reduces Flops and maintains or even \emph{improves} the model's performance at large-scale pretraining.

==> c_program.tex <==
%\section{Proposal: Hybrid convolutional Transformer architecture}
\section{Hybrid convolutional Transformer architecture}
\label{sec:hybrid}



\begin{figure}[h]
%\vspace{-0.7cm}
%\begin{minipage}{0.4\textwidth}
%\raggedleft
%    \includegraphics[trim={0cm 4cm 2cm 0cm},clip, width=7cm, left]{figures/code.pdf}
%\end{minipage}
\begin{minipage}{0.45\textwidth}
\raggedleft
\begin{lstlisting}[breaklines]
[BOS] a[0]=1; a[1]=-3; a[2]=2; a[3]=-2; a[4]=0; [SEP] int * func_1(int a[]){ int p_0 = 4; int l_7 = 2; ++a[l_7]; for (p_0 = 0; p_0 <= 2; p_0++) { a[p_0] = 0; for (int p_1 = 3; p_1 >= 2; p_1--) { a[p_1]--;} } return a; } [EOS]

[BOS] a[0]=-4; a[1]=1; a[2]=3; a[3]=0; a[4]=1; [SEP] int * func_1(int a[]) { int p_0 = 1; int l_9 = 1; a[l_9] = (0 * a[p_0]); return a; } [EOS]

[BOS] a[0]=0; a[1]=3; a[2]=-1; a[3]=4; a[4]=-2; [SEP] int * func_1(int a[]) { int p_0 = 0; int l_9 = 3; for (p_0 = 4; p_0 >= 3; p_0--) { a[p_0] = 0; a[p_0] = (a[l_9] * a[p_0]);} return a; }[EOS]
 
            ......
\end{lstlisting}
\end{minipage}
\hspace{\fill}
\begin{minipage}{0.5\textwidth}
\raggedright
  \includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=6cm, height=4.2cm]{figures/conv_ccode.pdf}
\end{minipage}
\vspace{-0.2cm}
\caption{Left: Example input sequences adapted from the restricted C dataset. Right: Performance of vanilla BERT vs. hybrid architecture with convolutional filter sizes (5, 10, 15). Error bars are standard deviations of 3 independent runs.}
\label{fig:cprog}
\vspace{-0.5cm}
\end{figure}




%\textbf{Proposal: Hybrid convolutional Transformer architecture.}
Our above findings suggest a natural modification to the Transformer architecture. Out of the two fundamental attention patterns---association and manipulation, only the latter depends on the positions of tokens in the sequence. Since this pattern appears crucial for LEGO, and perceivably for many symbolic reasoning tasks, it seems helpful to encode it directly into the architecture, rather than letting the model learn it indirectly from massive data. This is akin to the way convolutional layers directly encode relations between adjacent pixels in their architecture. 
%Since such ``local'' or convolutional attention patterns are likely valuable in virtually all natural language tasks, it is intriguing to also apply this idea to language models in general.

We instantiate this idea by implementing the a hybrid convolutional multi-head attention module, where we give precise details in Appendix~\ref{sec:conv-attn}. At a high-level, in each attention head, we apply the key, query and value linear transformations are applied not just to each token on its own, but to an outcome of a one-dimensional convolution along the temporal dimension of the input sequence. To avoid excessive amount of additional parameters, we adopt depth-wise convolutions~\cite{chollet2017xception}, i.e., one filter per input dimension. We are aware of existing extremely similar, popularized ideas in computer vision~\cite{dai2021coatnet,liu2021Swin, liu2022convnet} and natural language processing~\cite{jiang2020convbert, Cordonnier2020On}. We intend to provide evidential motivations for its use in reasoning tasks rather than to claim novelty. 


We evaluate this hybrid convolutional multi-head attention module on both LEGO and a more advanced symbolic reasoning task than LEGO --- learning to execute C programs. The details of both experiments can be found in Appendix~\ref{sec:conv-attn}. 
As a sanity check, on LEGO, modified BERT and ALBERT not only are capable of matching the performance of their pre-trained unmodified versions, but also avoid the shortcut solutions. 

For the task of learning to execute C programs, we use the restricted C dataset~\cite{chen2021latent} of $500$K programs written in C, each with initial values of input variables as well as final outcomes. We consider the task to predict the outcome given the initial values and the program. Here we convert each program and corresponding initial assignments into plain text and feed it to the model as the input sentence. Then we apply a linear classifier to the output representations, same as in LEGO. Figure~\ref{fig:cprog} shows that the convolutional architecture attains a significant performance advantage over the vanilla BERT on this task with less than $0.5\%$ extra parameters. We provide details in Appendix~\ref{sec:c-programs}.

%\subsection{Do pre-trained models generalize better, and for what reasons?}
%\begin{figure}[htb] 
%    \centering
%    \includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=14cm]{figures/mimicking_gen.pdf}
%    \caption{Mimicking association and manipulation heads closes the performance gap between pre-trained v.s. rand-init Transformers.}
%    \label{fig:pretrain}
%\end{figure}
%
%
%As seen in numerous recent works, the paradigm of pre-training a network on a large dataset followed by task-specific fine-tuning has been successful in achieving high accuracy in a variety of tasks ([refs]). Our next objective was to use our model as a testing ground for this paradigm. We do this by training the same architecture with either (a) random initialization or (b) initialization obtained by pre-training the network on language corpus (TODO: expand).
%
%We tested the effect of pre-training on the models performance in out-of-distribution generalization. Figure \ref{fig:pretrain} (left and center plots) shows that pre-training helps generalization in LEGO dramatically - the pre-trained model generalizes to longer sequences much better, and within a far smaller number of epochs, than the randomly initialized one. In what follows, we investigate the root causes for this advantage, and draw on our findings to suggest a modification to the Transformer architecture.
%
%
%
%It can be witnessed that Transformer models are capable of performing reasoning tasks to a certain extent (see discussion in Section~\ref{sec:discussion} below). Therefore, the success of the pre-trained model in generalizing to the LEGO reasoning task may lead one to postulate that those models have essentially “learned to reason”. However, we posit that this is not the case, and that instead their success is rooted in having learned certain fundamental attention patterns, which facilitate LEGO despite encompassing no “reasoning” capabilities. One may come up, however, with several other possible explanations for the advantage of pre-trained networks which are more straightforward. 
%
%At its basis, the LEGO task requires two fundamental types of information transfer, which we refer to as \emph{association} and \emph{manipulation}:
%\begin{itemize}
%  \item \emph{Manipulation/Assignment:} transferring a value from the right-hand to the left-hand side of the '=' within each clause. For example, to successfully process the clause ``$b=-a$'', the architecture must associate these particular occurrences of $a$ and $b$ with each other, in order to transfer the value of $a$ (after applying to it the group element $-1$) into $b$. 
%  \item \emph{Association:} encoding long range dependencies that transfer a value between two occurrences of the same variable. For example, if the input contains the two clauses ``$a=1$'' and ``$b=-a$'' (with arbitrary separation between them), the architecture must associate the two occurrences of the variable $a$ in order to correctly set $b$ to $-1$.
%\end{itemize}
%
%\begin{figure}[t]
%    \centering
%    \includegraphics[trim={3cm 0cm 0cm 0cm},clip, width=13cm]{figures/attention_eyeball.pdf}
%    \caption{Visualization of attention maps from a pre-trained but not yet fine-tuned BERT model's first layer. On a LEGO input sequence unseen by the model, certain heads have already managed to implement a manipulations operator (left), while the other implements an association operators (right). We provide a complete visualization for all attention maps of the pre-trained BERT in the Appendix.}
%    \label{fig:attention_heads}
%\end{figure}
%
%
%Notice that the two types correspond to two fundamental attention patterns. Association corresponds to a purely global attention pattern, which is completely reliant on the \emph{content} of the tokens while being oblivious to their \emph{position} in the input sequence. Assignment, in contrast, corresponds to a purely local attention pattern, where nearby positions attend to each other. The LEGO task crystallizes the roles of these fundamental patterns, as explained above, so it is natural to ask whether they are indeed manifested in the Transformer attention heads in practice.
%
%The answer turns out to be positive. Fig.~\ref{fig:attention_heads} shows 2 exemplar attention heads in the pre-trained BERT, upon seeing an input LEGO sequence without any fine-tuning ( visualization of the remaining attention heads is provided in the Appendix) . We observe that one can categorize all attention heads of the pre-trained BERT essentially into to three types: ``association heads'' where each token attends to all other occurrences of the same token in the input sequence; ``manipulation heads'' where each token attends to the tokens immediately before and after it in the sequence; and ``blank heads'', which do not exhibit any clear attention pattern at all. This leads us to posit that the pre-trained model had already learned how to realize the association and manipulation attention patterns, which arise in many natural language tasks. The fact that these patterns are apparently already encoded in the pre-trained models may explain their ability to generalize on the LEGO task previously unseen by them, irrespective of any reasoning capacity they may or may not possess. As for the ``blank'' attention heads, they possibly encode other attention patterns learned during pre-training, that do not arise in LEGO.
%
%To summarize, we will consider the following possible explanations in increasing order of "complexity":
%\begin{enumerate} [topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex, leftmargin=5ex]
%\item
%In the pre-trained model there are likely to be attention heads of the form $Q_V = Q_K^T$, meaning that the operation of performing association between identical tokens is already integrated in the network. 
%\item
%The attention heads at initialization are already calibrated to 'interpret' the positional encoding.
%\item
%The pre-trained network is already able to recognize and "make sense of" several tokens, such as the '=' sign or the '-' sign, and interpret those symbols in the right way.
%\item
%The pre-trained network has obtained, to some extent, an innate ability to "reason".
%\end{enumerate}
%
%First of all, to exclude the third explanation we simply used different tokens in place of the symbols ('=', '+' and '-') and observed that the model has the same performance both in terms of training speed and generalization. It is not clear how to check the role of the fourth explanation directly, but we can get indirect evidence by showing that the other explanations fully account for the advantage of pre-training. 
%
%In order to test the extent of effect of the first two explanations, instead of pre-training the model on the language corpus, we propose a superficial Mimicking procedure whose goal is to give rise to the two aforementioned types of attention heads thereby mimicking the desired effect of pre-training. 
%
%
%
%\section{Proposal: convolutional attentions as positional encoding}
%
%The foregoing discussion suggests a natural modification to the Transformer architecture. Since token positions in the sequence are only used in LEGO to attend to adjacent tokens (in the manipulation attention pattern, while the association attention pattern is oblivious to positions), it appears helpful to encode this pattern directly in the architecture, rather than having the model learn it using positional encodings. This is akin to the way convolutional layers directly encode relations between adjacent pixels in their architecture. Since such ``local'' or convolutional attention patterns are likely valuable in virtually all natural language tasks, it is intriguing to also apply this idea to lanaguage models in general.
%
%We instantiate this idea by implementing the following hybrid between convolutional and Transformer architectures. In each attention head, the key, query and value linear transformations are applied not just to each token on its own, but also the tokens immediately before and after it in the sequence (this can be thought of as a one-dimensional convolution filter of size $3$ over the sequence). The same modification is also applied to the final linear transformation on the concatenated outputs of the attention heads. 
%
%More formally, recall that the multi-head attention layer in the original Transformer model with sequence length $n$, model dimension $d$ and number of heads $h$ is given by,
%\begin{align*}
%    \mathrm{MultiHead}(Q,K,V) &:= O\cdot W^O \\
%    \text{where} \;\;\;\; O &:= \mathrm{Concat}(\{\mathrm{Attention}(Q\cdot W_i^Q, K\cdot W_i^K, V\cdot W_i^V):i=1,\ldots,h\}) ,
%\end{align*}
%
%
%where $Q,K,V\in\R^{n\times d}$ are the query, key and value embeddings given as input to the attention layer, and $W_i^Q,W_i^K,W_i^V\in\R^{d\times\tfrac{d}{h}}$, $W^O\in\R^{d\times d}$ are the learned linear operators.
%%
%To define our hybrid architecture, for any matrix $M\in\R^{n\times d}$, let $\bar M\in\R^{n\times 3d}$ denote the matrix in which each row $j=1,\ldots,n$ contains the horizontal concatenation of rows $j-1,j,j+1$ of $M$, where by convention we define rows $j=-1$ and $j=n+1$ to be zeros. Our hybrid multi-head attention operation is now given by,
%
%\begin{align*}
%    \mathrm{MultiHead}(Q,K,V) &:= \bar O\cdot W^O \\
%    \text{where} \;\;\;\; O &:= \mathrm{Concat}(\{\mathrm{Attention}(\bar Q\cdot W_i^Q, \bar K\cdot W_i^K, \bar V\cdot W_i^V):i=1,\ldots,h\}) ,
%\end{align*}
%where this time the learned linear operators have their row-dimension multiplied by $3$, i.e.,  $W_i^Q,W_i^K,W_i^V\in\R^{3d\times\tfrac{d}{h}}$ and $W^O\in\R^{3d\times d}$.
%
%\subsection{Sanity check: convolutional Transformers for LEGO}
%\begin{figure}[H]
%    \centering
%    \begin{subfigure}{\textwidth}
%     \begin{minipage}[r]{0.05\textwidth}
%     \caption{}
%  \end{minipage}
%  \begin{minipage}[l]{0.95\textwidth}
%    \includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=13cm]{figures/conv_shortcut.pdf}
%    \end{minipage}
%    \end{subfigure}
%    %\vspace{0.01cm}
%    \hrule
%    \vspace{0.05cm}
%\begin{subfigure}{\textwidth}
%     \begin{minipage}[r]{0.05\textwidth}
%     \caption{}
%  \end{minipage}
%  \begin{minipage}[l]{0.95\textwidth}
%    \includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=13cm]{figures/conv_gen.pdf}
%    \end{minipage}
%    \end{subfigure}
%    \caption{Solving LEGO using Convolutional BERT and ALBERT. With trained from random initialization, convolutional attention modules enable Transformers to (a) avoid shortcut solutions and to (b) match the learning speed as well as final generaliztation performance of their pre-trained/mimicking counterparts, given the same hyperparameters. Here we use depth-wise convolution of kernel size $5$ for all plots.}
%    \label{fig:shortcut-rand}
%\end{figure}


%\subsection{Bonus: learning to execute C programs}

%Now that we have verified the effectiveness of convolutional attention architecture for learning symbolic logic and reasoning, we evaluate it on a closely related but more sophisticated, real world task\textemdash learning to execute C programs.




==> conv.tex <==
To cite: \cite{Cordonnier2020On}.

==> discussion.tex <==
%\subsection{GPT-3}
\newpage
\section{Experiments with GPT-3}

We tried a zero shot learning with GPT-3 on the OpenAI website\footnote{\url{https://beta.openai.com/playground/p/default-grammar}}. The red text is the completion given by the ``text-davinci-002'' model with Temperature $=0$ and Top P $=0$:

\texttt{{a=+1; b=-a; c=-b; d=+c; e=+d; f=-e; g=-f; h=+g; i=+h; j=-i; k=-j; l=+k; m=+l; n=-m; o=+n; p=-o; q=-p; r=+q; s=+r; t=-s; u=+t; v=-u; w=-v; x=+w; y=+x; z=-y;
\linebreak
\linebreak
a=1; b=-1; c=1; d=1; e=\color{red}1; f=-1; g=-1; h=1; i=1; j=-1; k=-1; l=1; m=1; n=-1; o=1; p=-1; q=-1; r=1; s=1; t=-1; u=1; v=-1; w=-1; x=1; y=1; z=-1}}

Note that the variable \texttt{g} is computed incorrectly (it is the first variable computed incorrectly in the chain of variables).


Next, we added the text ``\texttt{Compute the variables from left to right:}'' in front of the previous prompt:

\texttt{{Compute the variables from left to right:
\linebreak
\linebreak
a=+1; b=-a; c=-b; d=+c; e=+d; f=-e; g=-f; h=+g; i=+h; j=-i; k=-j; l=+k; m=+l; n=-m; o=+n; p=-o; q=-p; r=+q; s=+r; t=-s; u=+t; v=-u; w=-v; x=+w; y=+x; z=-y;
\linebreak
\linebreak
a=1; b=-1; c=1; d=1; e=\color{red}1; f=-1; g=1; h=1; i=1; j=-1; k=1; l=1; m=1; n=-1; o=1; p=-1; q=1; r=1; s=-1; t=1; u=1; v=-1; w=1; x=1; y=-1; z=1}}

This improves the performance but the variable \texttt{o} is computed incorrectly (it is the first variable computed incorrectly in the chain of variables). Adding example computations (few show learning) did not help to improve the performance.

There are 3 significant differences between our setup and GPT-3. First, GPT-3 doesn't require any finetuning or training on our synthetic reasoning task. Second, the architecture of GPT-3 is entirely a decoder-based architecture with a causal attention mask while all our architectures have bidirectional attention. Third, the text generation done by GPT-3 proceeds in a loop by executing the model and generating tokens in a sequential manner. Our models generate the token embeddings all at once. This makes the generation process of GPT-3 more powerful as it doesn't need to compute the values of the variables all at once but might do that sequentially.


\iffalse
\begin{figure}[H]
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=14cm]{figures/openai.jpg}
\caption{The colored text is the completion given by GPT-3 for the prompt.}
\label{fig:gpt3}
\end{figure}

%\subsection{GitHub Copilot}
\begin{figure}[H]
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=14cm]{figures/copilot.jpg}
\caption{The shaded text is the completion given by GitHub Copilot for the prompt.}
\label{fig:gpt3}
\end{figure}

\paragraph{Drawbacks}
The drawbacks are twofold. First, both GPT-3 and GitHub Copilot requires effort to design the prompt (requires prompt tuning). For similar prompts the outcomes can be very different. Second, even for a fixed outcome, the outcome might be randomized (depending on the text generation procedure).


{\color{red} SG: may be also add an example with tokens like $+\to floo$, $-\to boo$ few short learning -- it would be interesting both if it succeeds with $~10$ examples or fails


Arturs: even this doesn't work:


\begin{figure}[H]
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=14cm]{figures/copilot2.jpg}
\caption{The shaded text is the completion given by GitHub Copilot for the prompt.}
\label{fig:gpt3}
\end{figure}
}
\fi

==> longer_seq.tex <==
\section{Generalization to longer sequences}
\begin{figure}[H]
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=14cm]{figures/n=2_pretrained_vs_randinit.pdf}
\caption{Predicting longer sequences. We finetune/train  BERT and ALBERT models that are pre-trained/random-initialized on input sequences consisting of 12 variables in total. During training, we only provide label information on the first 6 variables (\#0 to \#5) along the chain. However, For testing, we instead evaluate the models' predictions on all 12 variables (\#0 to \#11) of hold-out test sequences.}
\label{fig:gen_longer_seq}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

